The Stellar Populations and Rest-Frame Colors of Star-Forming Galaxies at $z \approx 8$: Exploring the Impact of Filter Choice and Star Formation History Assumption with JADES

Our understanding of the physical properties of star-forming galaxies during the Epoch of Reionization (EoR, at $z > 6$) suffers from degeneracies among the apparent properties of the stars, the nebular gas, and the dust. These degeneracies are most prominent with photometry, which has insufficient (1) spectral resolution and (2) rest-frame spectral coverage. We explore ways to break these degeneracies with a sample of $N = 22$ high-redshift star-forming galaxies at $7 < z_{\mathrm{phot}} \leq 9$, using some of the deepest existing imaging from JWST/NIRCam and JWST/MIRI with JADES. Key to this study is the imaging from JWST/MIRI at $7.7\ \mu\mathrm{m}$, which provides coverage of the rest-frame $I$-band at the observed redshifts. We infer stellar population properties and rest-frame colors using a variety of filter sets and star formation history assumptions to explore the impact of these choices. Evaluating these quantities both with and without the $7.7\ \mu\mathrm{m}$ data point shows that dense spectral coverage with JWST/NIRCam (eight or more filters, including at least one medium-band) can compensate for lacking the rest-frame $I$-band coverage for the vast majority ($\approx 80\%$) of our sample. Furthermore, these galaxy properties are most consistently determined by assuming the delayed-tau star formation history, which provides the smallest offsets and scatters around these offsets when including JWST/MIRI. Within extragalactic surveys like JADES and CEERS, our findings suggest that robust characterization of the stellar population properties and rest-frame colors for high-redshift star-forming galaxies is possible with JWST/NIRCam alone at $z \approx 8$.

==> stellar_populations_table.tex <==
% Derived Stellar Population Property \\

% SFH & GalaxyID & logStellarMass & logMassWeightedAge & logSFR10 & logSpecificSFR10 & logRestOpticalEquivalentWidth \\

% CSFH & $14647$ & $7.451^{+0.110}_{-0.089}$ & $6.576^{+0.250}_{-0.302}$ & $0.407^{+0.069}_{-0.061}$ & $-7.000^{+0.000}_{-0.127}$ & $3.294^{+0.144}_{-0.047}$ \\
% CSFH & $21468$ & $7.940^{+0.219}_{-0.204}$ & $7.131^{+0.283}_{-0.264}$ & $0.501^{+0.079}_{-0.078}$ & $-7.432^{+0.264}_{-0.283}$ & $3.073^{+0.056}_{-0.056}$ \\
% CSFH & $25526$ & $7.806^{+0.088}_{-0.075}$ & $6.698^{+0.110}_{-0.177}$ & $0.765^{+0.054}_{-0.048}$ & $-7.000^{+0.000}_{-0.110}$ & $3.309^{+0.077}_{-0.040}$ \\
% CSFH & $27503$ & $8.111^{+0.101}_{-0.106}$ & $6.840^{+0.123}_{-0.226}$ & $0.964^{+0.055}_{-0.056}$ & $-7.141^{+0.141}_{-0.123}$ & $3.224^{+0.049}_{-0.047}$ \\
% CSFH & $30333$ & $7.860^{+0.060}_{-0.089}$ & $6.834^{+0.056}_{-0.063}$ & $0.726^{+0.046}_{-0.074}$ & $-7.135^{+0.063}_{-0.056}$ & $3.256^{+0.026}_{-0.028}$ \\
% CSFH & $37458$ & $7.629^{+0.135}_{-0.074}$ & $6.883^{+0.189}_{-0.104}$ & $0.440^{+0.041}_{-0.051}$ & $-7.184^{+0.104}_{-0.189}$ & $3.223^{+0.031}_{-0.041}$ \\
% CSFH & $57378$ & $8.346^{+0.112}_{-0.123}$ & $7.124^{+0.153}_{-0.168}$ & $0.923^{+0.057}_{-0.063}$ & $-7.425^{+0.168}_{-0.153}$ & $3.083^{+0.052}_{-0.043}$ \\
% CSFH & $66293$ & $9.001^{+0.081}_{-0.081}$ & $7.056^{+0.106}_{-0.099}$ & $1.641^{+0.077}_{-0.085}$ & $-7.357^{+0.099}_{-0.105}$ & $2.820^{+0.056}_{-0.054}$ \\
% CSFH & $164055$ & $7.515^{+0.199}_{-0.154}$ & $6.883^{+0.302}_{-0.261}$ & $0.306^{+0.084}_{-0.102}$ & $-7.184^{+0.184}_{-0.302}$ & $3.221^{+0.090}_{-0.102}$ \\
% CSFH & $165595$ & $8.371^{+0.087}_{-0.084}$ & $7.189^{+0.111}_{-0.098}$ & $0.879^{+0.051}_{-0.054}$ & $-7.490^{+0.098}_{-0.111}$ & $3.043^{+0.032}_{-0.035}$ \\
% CSFH & $173624$ & $7.908^{+0.082}_{-0.082}$ & $6.860^{+0.098}_{-0.074}$ & $0.733^{+0.065}_{-0.066}$ & $-7.161^{+0.074}_{-0.098}$ & $3.251^{+0.029}_{-0.034}$ \\
% CSFH & $173679$ & $9.102^{+0.182}_{-0.189}$ & $7.807^{+0.248}_{-0.232}$ & $0.981^{+0.110}_{-0.099}$ & $-8.108^{+0.232}_{-0.248}$ & $2.670^{+0.088}_{-0.067}$ \\
% CSFH & $174121$ & $7.860^{+0.073}_{-0.054}$ & $6.409^{+0.125}_{-0.264}$ & $0.860^{+0.072}_{-0.054}$ & $-7.000^{+0.000}_{+0.000}$ & $3.548^{+0.073}_{-0.074}$ \\
% CSFH & $174693$ & $8.313^{+0.235}_{-0.238}$ & $7.660^{+0.337}_{-0.342}$ & $0.346^{+0.122}_{-0.109}$ & $-7.961^{+0.342}_{-0.337}$ & $2.896^{+0.070}_{-0.060}$ \\
% CSFH & $175729$ & $8.106^{+0.166}_{-0.172}$ & $7.119^{+0.235}_{-0.249}$ & $0.685^{+0.099}_{-0.091}$ & $-7.420^{+0.249}_{-0.235}$ & $3.127^{+0.080}_{-0.066}$ \\
% CSFH & $175837$ & $8.538^{+0.217}_{-0.231}$ & $7.503^{+0.370}_{-0.385}$ & $0.705^{+0.237}_{-0.176}$ & $-7.804^{+0.385}_{-0.370}$ & $2.880^{+0.082}_{-0.080}$ \\
% CSFH & $177322$ & $7.860^{+0.252}_{-0.215}$ & $7.019^{+0.334}_{-0.319}$ & $0.530^{+0.086}_{-0.090}$ & $-7.320^{+0.319}_{-0.333}$ & $3.121^{+0.078}_{-0.067}$ \\
% CSFH & $179485$ & $8.806^{+0.133}_{-0.120}$ & $7.392^{+0.205}_{-0.182}$ & $1.113^{+0.075}_{-0.087}$ & $-7.693^{+0.182}_{-0.205}$ & $2.860^{+0.041}_{-0.050}$ \\
% CSFH & $180446$ & $8.466^{+0.107}_{-0.177}$ & $8.140^{+0.154}_{-0.267}$ & $0.031^{+0.108}_{-0.075}$ & $-8.441^{+0.267}_{-0.154}$ & $2.719^{+0.050}_{-0.050}$ \\
% CSFH & $300287$ & $8.067^{+0.077}_{-0.074}$ & $6.404^{+0.088}_{-0.128}$ & $1.067^{+0.077}_{-0.074}$ & $-7.000^{+0.000}_{+0.000}$ & $2.730^{+0.103}_{-0.101}$ \\
% CSFH & $300391$ & $7.882^{+0.083}_{-0.052}$ & $6.543^{+0.185}_{-0.130}$ & $0.878^{+0.051}_{-0.048}$ & $-7.000^{+0.000}_{-0.029}$ & $3.394^{+0.073}_{-0.068}$ \\
% CSFH & $380203$ & $7.545^{+0.148}_{-0.077}$ & $6.297^{+0.464}_{-0.330}$ & $0.541^{+0.089}_{-0.075}$ & $-7.000^{+0.000}_{-0.062}$ & $3.088^{+0.262}_{-0.082}$ \\

% DtSFH & $14647$ & $7.525^{+0.084}_{-0.104}$ & $6.516^{+0.430}_{-0.457}$ & $0.429^{+0.129}_{-0.080}$ & $-7.000^{+0.000}_{-0.214}$ & $3.341^{+0.147}_{-0.067}$ \\
% DtSFH & $21468$ & $7.970^{+0.200}_{-0.187}$ & $7.242^{+0.270}_{-0.271}$ & $0.498^{+0.072}_{-0.070}$ & $-7.465^{+0.232}_{-0.252}$ & $3.097^{+0.058}_{-0.058}$ \\
% DtSFH & $25526$ & $7.802^{+0.077}_{-0.068}$ & $6.711^{+0.143}_{-0.159}$ & $0.730^{+0.045}_{-0.035}$ & $-7.057^{+0.055}_{-0.089}$ & $3.367^{+0.055}_{-0.048}$ \\
% DtSFH & $27503$ & $8.173^{+0.094}_{-0.095}$ & $6.928^{+0.162}_{-0.172}$ & $0.966^{+0.071}_{-0.068}$ & $-7.200^{+0.118}_{-0.131}$ & $3.256^{+0.062}_{-0.052}$ \\
% DtSFH & $30333$ & $7.902^{+0.090}_{-0.091}$ & $6.881^{+0.176}_{-0.116}$ & $0.727^{+0.057}_{-0.093}$ & $-7.165^{+0.077}_{-0.139}$ & $3.295^{+0.042}_{-0.053}$ \\
% DtSFH & $37458$ & $7.710^{+0.117}_{-0.102}$ & $7.052^{+0.169}_{-0.161}$ & $0.409^{+0.032}_{-0.033}$ & $-7.299^{+0.127}_{-0.148}$ & $3.224^{+0.043}_{-0.039}$ \\
% DtSFH & $57378$ & $8.355^{+0.101}_{-0.095}$ & $7.232^{+0.146}_{-0.136}$ & $0.903^{+0.052}_{-0.068}$ & $-7.456^{+0.120}_{-0.136}$ & $3.117^{+0.043}_{-0.042}$ \\
% DtSFH & $66293$ & $9.062^{+0.076}_{-0.073}$ & $7.086^{+0.094}_{-0.077}$ & $1.726^{+0.087}_{-0.089}$ & $-7.327^{+0.064}_{-0.081}$ & $2.874^{+0.048}_{-0.055}$ \\
% DtSFH & $164055$ & $7.571^{+0.152}_{-0.128}$ & $7.005^{+0.235}_{-0.276}$ & $0.304^{+0.083}_{-0.080}$ & $-7.260^{+0.194}_{-0.204}$ & $3.247^{+0.071}_{-0.078}$ \\
% DtSFH & $165595$ & $8.378^{+0.087}_{-0.086}$ & $7.274^{+0.122}_{-0.116}$ & $0.882^{+0.048}_{-0.051}$ & $-7.494^{+0.105}_{-0.112}$ & $3.085^{+0.034}_{-0.035}$ \\
% DtSFH & $173624$ & $7.924^{+0.100}_{-0.099}$ & $6.932^{+0.162}_{-0.155}$ & $0.709^{+0.060}_{-0.049}$ & $-7.203^{+0.108}_{-0.132}$ & $3.279^{+0.048}_{-0.045}$ \\
% DtSFH & $173679$ & $9.102^{+0.131}_{-0.138}$ & $7.884^{+0.177}_{-0.183}$ & $1.005^{+0.085}_{-0.088}$ & $-8.099^{+0.182}_{-0.172}$ & $2.692^{+0.066}_{-0.050}$ \\
% DtSFH & $174121$ & $7.933^{+0.093}_{-0.074}$ & $6.329^{+0.288}_{-0.486}$ & $0.923^{+0.097}_{-0.074}$ & $-7.000^{+0.000}_{-0.017}$ & $3.566^{+0.056}_{-0.091}$ \\
% DtSFH & $174693$ & $8.287^{+0.189}_{-0.207}$ & $7.706^{+0.264}_{-0.292}$ & $0.376^{+0.093}_{-0.083}$ & $-7.907^{+0.283}_{-0.261}$ & $2.936^{+0.065}_{-0.057}$ \\
% DtSFH & $175729$ & $8.101^{+0.159}_{-0.159}$ & $7.187^{+0.243}_{-0.263}$ & $0.681^{+0.083}_{-0.083}$ & $-7.415^{+0.219}_{-0.223}$ & $3.166^{+0.078}_{-0.067}$ \\
% DtSFH & $175837$ & $8.525^{+0.238}_{-0.231}$ & $7.529^{+0.352}_{-0.355}$ & $0.762^{+0.202}_{-0.170}$ & $-7.740^{+0.335}_{-0.352}$ & $2.934^{+0.118}_{-0.080}$ \\
% DtSFH & $177322$ & $7.903^{+0.236}_{-0.202}$ & $7.113^{+0.339}_{-0.314}$ & $0.530^{+0.085}_{-0.081}$ & $-7.352^{+0.243}_{-0.311}$ & $3.130^{+0.072}_{-0.065}$ \\
% DtSFH & $179485$ & $8.836^{+0.127}_{-0.119}$ & $7.521^{+0.192}_{-0.186}$ & $1.107^{+0.072}_{-0.077}$ & $-7.729^{+0.178}_{-0.192}$ & $2.866^{+0.044}_{-0.046}$ \\
% DtSFH & $180446$ & $8.316^{+0.173}_{-0.211}$ & $7.886^{+0.229}_{-0.312}$ & $0.176^{+0.186}_{-0.140}$ & $-8.113^{+0.327}_{-0.274}$ & $2.756^{+0.092}_{-0.106}$ \\
% DtSFH & $300287$ & $8.066^{+0.055}_{-0.059}$ & $6.464^{+0.161}_{-0.133}$ & $1.054^{+0.054}_{-0.059}$ & $-7.000^{+0.000}_{-0.019}$ & $2.674^{+0.112}_{-0.093}$ \\
% DtSFH & $300391$ & $7.940^{+0.086}_{-0.067}$ & $6.548^{+0.204}_{-0.597}$ & $0.906^{+0.060}_{-0.048}$ & $-7.001^{+0.001}_{-0.079}$ & $3.436^{+0.108}_{-0.058}$ \\
% DtSFH & $380203$ & $7.577^{+0.094}_{-0.083}$ & $6.166^{+0.632}_{-0.350}$ & $0.537^{+0.083}_{-0.090}$ & $-7.000^{+0.000}_{-0.108}$ & $3.247^{+0.136}_{-0.207}$ \\

% ContSFH & $14647$ & $8.281^{+0.089}_{-0.085}$ & $8.386^{+0.083}_{-0.055}$ & $0.417^{+0.169}_{-0.063}$ & $-7.829^{+0.111}_{-0.120}$ & $3.167^{+0.066}_{-0.051}$ \\
% ContSFH & $21468$ & $8.407^{+0.100}_{-0.116}$ & $8.188^{+0.068}_{-0.083}$ & $0.443^{+0.132}_{-0.107}$ & $-7.955^{+0.170}_{-0.164}$ & $2.973^{+0.081}_{-0.084}$ \\
% ContSFH & $25526$ & $8.286^{+0.131}_{-0.097}$ & $8.138^{+0.133}_{-0.178}$ & $0.738^{+0.056}_{-0.050}$ & $-7.554^{+0.108}_{-0.113}$ & $3.228^{+0.036}_{-0.038}$ \\
% ContSFH & $27503$ & $8.193^{+0.174}_{-0.120}$ & $7.861^{+0.276}_{-0.793}$ & $0.963^{+0.062}_{-0.063}$ & $-7.229^{+0.134}_{-0.192}$ & $3.181^{+0.042}_{-0.044}$ \\
% ContSFH & $30333$ & $8.160^{+0.063}_{-0.067}$ & $8.096^{+0.069}_{-0.095}$ & $0.516^{+0.062}_{-0.082}$ & $-7.653^{+0.096}_{-0.090}$ & $3.069^{+0.045}_{-0.054}$ \\
% ContSFH & $37458$ & $7.529^{+0.094}_{-0.052}$ & $7.217^{+0.415}_{-0.947}$ & $0.839^{+0.024}_{-0.020}$ & $-6.686^{+0.053}_{-0.099}$ & $3.660^{+0.014}_{-0.020}$ \\
% ContSFH & $57378$ & $8.577^{+0.083}_{-0.080}$ & $7.859^{+0.176}_{-0.227}$ & $0.881^{+0.077}_{-0.082}$ & $-7.701^{+0.118}_{-0.114}$ & $3.047^{+0.049}_{-0.047}$ \\
% ContSFH & $66293$ & $9.650^{+0.094}_{-0.113}$ & $8.359^{+0.026}_{-0.035}$ & $1.691^{+0.144}_{-0.140}$ & $-7.940^{+0.138}_{-0.124}$ & $2.870^{+0.086}_{-0.086}$ \\
% ContSFH & $164055$ & $8.109^{+0.105}_{-0.089}$ & $8.328^{+0.064}_{-0.276}$ & $0.337^{+0.248}_{-0.068}$ & $-7.590^{+0.126}_{-0.334}$ & $3.232^{+0.088}_{-0.057}$ \\
% ContSFH & $165595$ & $9.684^{+0.236}_{-0.186}$ & $8.220^{+0.046}_{-0.070}$ & $1.477^{+0.241}_{-0.211}$ & $-8.209^{+0.154}_{-0.152}$ & $2.499^{+0.069}_{-0.074}$ \\
% ContSFH & $173624$ & $8.220^{+0.088}_{-0.103}$ & $7.801^{+0.154}_{-0.219}$ & $0.855^{+0.084}_{-0.075}$ & $-7.355^{+0.139}_{-0.143}$ & $3.302^{+0.044}_{-0.046}$ \\
% ContSFH & $173679$ & $9.418^{+0.142}_{-0.121}$ & $8.278^{+0.024}_{-0.035}$ & $0.855^{+0.063}_{-0.097}$ & $-8.566^{+0.125}_{-0.171}$ & $2.505^{+0.078}_{-0.129}$ \\
% ContSFH & $174121$ & $8.880^{+0.070}_{-0.094}$ & $8.363^{+0.073}_{-0.051}$ & $1.116^{+0.053}_{-0.062}$ & $-7.759^{+0.114}_{-0.102}$ & $3.284^{+0.026}_{-0.028}$ \\
% ContSFH & $174693$ & $8.632^{+0.098}_{-0.096}$ & $8.265^{+0.066}_{-0.174}$ & $0.289^{+0.151}_{-0.123}$ & $-8.340^{+0.217}_{-0.195}$ & $2.815^{+0.098}_{-0.097}$ \\
% ContSFH & $175729$ & $8.483^{+0.115}_{-0.121}$ & $8.165^{+0.067}_{-0.117}$ & $0.619^{+0.123}_{-0.142}$ & $-7.834^{+0.154}_{-0.245}$ & $3.043^{+0.086}_{-0.105}$ \\
% ContSFH & $175837$ & $8.310^{+0.620}_{-0.101}$ & $7.526^{+0.827}_{-0.410}$ & $0.948^{+0.070}_{-0.408}$ & $-7.315^{+0.052}_{-1.052}$ & $3.011^{+0.060}_{-0.067}$ \\
% ContSFH & $177322$ & $8.474^{+0.117}_{-0.117}$ & $8.247^{+0.064}_{-0.105}$ & $0.517^{+0.146}_{-0.121}$ & $-7.937^{+0.194}_{-0.226}$ & $3.034^{+0.084}_{-0.073}$ \\
% ContSFH & $179485$ & $9.195^{+0.056}_{-0.062}$ & $8.252^{+0.045}_{-0.049}$ & $1.119^{+0.097}_{-0.091}$ & $-8.073^{+0.126}_{-0.121}$ & $2.849^{+0.058}_{-0.074}$ \\
% ContSFH & $180446$ & $8.529^{+0.287}_{-0.112}$ & $8.300^{+0.058}_{-0.444}$ & $-0.011^{+0.443}_{-0.195}$ & $-8.492^{+0.404}_{-0.394}$ & $2.489^{+0.252}_{-0.143}$ \\
% ContSFH & $300287$ & $9.008^{+0.045}_{-0.079}$ & $8.472^{+0.061}_{-0.114}$ & $1.261^{+0.091}_{-0.141}$ & $-7.741^{+0.062}_{-0.083}$ & $2.479^{+0.047}_{-0.049}$ \\
% ContSFH & $300391$ & $8.378^{+0.176}_{-0.075}$ & $7.758^{+0.322}_{-0.507}$ & $0.863^{+0.059}_{-0.047}$ & $-7.523^{+0.082}_{-0.137}$ & $3.141^{+0.118}_{-0.031}$ \\
% ContSFH & $380203$ & $8.507^{+0.175}_{-0.132}$ & $8.251^{+0.070}_{-0.136}$ & $0.678^{+0.110}_{-0.126}$ & $-7.817^{+0.168}_{-0.277}$ & $2.835^{+0.045}_{-0.055}$ \\

% BurstySFH & $14647$ & $7.850^{+0.211}_{-0.208}$ & $8.039^{+0.233}_{-0.689}$ & $0.722^{+0.077}_{-0.115}$ & $-7.163^{+0.292}_{-0.233}$ & $3.477^{+0.054}_{-0.113}$ \\
% BurstySFH & $21468$ & $7.791^{+0.210}_{-0.123}$ & $7.151^{+0.373}_{-0.310}$ & $0.455^{+0.114}_{-0.113}$ & $-7.350^{+0.164}_{-0.215}$ & $3.055^{+0.084}_{-0.089}$ \\
% BurstySFH & $25526$ & $8.502^{+0.122}_{-0.137}$ & $8.327^{+0.042}_{-0.073}$ & $0.860^{+0.067}_{-0.060}$ & $-7.628^{+0.154}_{-0.161}$ & $3.352^{+0.048}_{-0.043}$ \\
% BurstySFH & $27503$ & $8.083^{+0.087}_{-0.075}$ & $7.043^{+0.352}_{-0.270}$ & $0.931^{+0.133}_{-0.092}$ & $-7.150^{+0.137}_{-0.121}$ & $3.222^{+0.093}_{-0.074}$ \\
% BurstySFH & $30333$ & $8.659^{+0.109}_{-0.100}$ & $7.509^{+0.408}_{-0.276}$ & $0.906^{+0.146}_{-0.163}$ & $-7.755^{+0.164}_{-0.187}$ & $2.771^{+0.051}_{-0.068}$ \\
% BurstySFH & $37458$ & $7.763^{+0.128}_{-0.147}$ & $7.234^{+0.385}_{-0.175}$ & $0.434^{+0.071}_{-0.070}$ & $-7.322^{+0.122}_{-0.127}$ & $3.208^{+0.045}_{-0.051}$ \\
% BurstySFH & $57378$ & $8.034^{+0.039}_{-0.044}$ & $6.913^{+0.487}_{-0.105}$ & $0.693^{+0.075}_{-0.051}$ & $-7.344^{+0.072}_{-0.032}$ & $3.028^{+0.049}_{-0.034}$ \\
% BurstySFH & $66293$ & $9.737^{+0.074}_{-0.072}$ & $7.124^{+0.300}_{-0.123}$ & $2.408^{+0.148}_{-0.130}$ & $-7.336^{+0.184}_{-0.153}$ & $2.910^{+0.032}_{-0.035}$ \\
% BurstySFH & $164055$ & $7.535^{+0.051}_{-0.096}$ & $6.940^{+0.516}_{-0.183}$ & $0.477^{+0.183}_{-0.091}$ & $-7.062^{+0.216}_{-0.084}$ & $3.312^{+0.105}_{-0.047}$ \\
% BurstySFH & $165595$ & $8.463^{+0.088}_{-0.091}$ & $7.587^{+0.299}_{-0.313}$ & $0.843^{+0.113}_{-0.131}$ & $-7.617^{+0.105}_{-0.127}$ & $2.998^{+0.064}_{-0.076}$ \\
% BurstySFH & $173624$ & $8.723^{+0.146}_{-0.136}$ & $7.709^{+0.277}_{-0.257}$ & $0.824^{+0.102}_{-0.100}$ & $-7.898^{+0.118}_{-0.136}$ & $2.854^{+0.035}_{-0.040}$ \\
% BurstySFH & $173679$ & $9.361^{+0.114}_{-0.130}$ & $8.173^{+0.133}_{-0.276}$ & $0.861^{+0.181}_{-0.249}$ & $-8.497^{+0.270}_{-0.320}$ & $2.396^{+0.114}_{-0.148}$ \\
% BurstySFH & $174121$ & $7.982^{+0.203}_{-0.112}$ & $7.296^{+0.651}_{-0.882}$ & $1.203^{+0.048}_{-0.054}$ & $-6.771^{+0.132}_{-0.245}$ & $3.628^{+0.032}_{-0.045}$ \\
% BurstySFH & $174693$ & $8.281^{+0.297}_{-0.263}$ & $7.927^{+0.290}_{-0.651}$ & $0.409^{+0.156}_{-0.132}$ & $-7.847^{+0.319}_{-0.408}$ & $2.918^{+0.081}_{-0.093}$ \\
% BurstySFH & $175729$ & $8.368^{+0.141}_{-0.187}$ & $8.233^{+0.162}_{-0.232}$ & $0.512^{+0.115}_{-0.080}$ & $-7.840^{+0.199}_{-0.174}$ & $2.979^{+0.080}_{-0.066}$ \\
% BurstySFH & $175837$ & $8.365^{+0.233}_{-0.285}$ & $7.740^{+0.312}_{-0.545}$ & $0.723^{+0.147}_{-0.149}$ & $-7.624^{+0.373}_{-0.351}$ & $2.899^{+0.089}_{-0.085}$ \\
% BurstySFH & $177322$ & $7.940^{+0.207}_{-0.216}$ & $8.147^{+0.167}_{-0.949}$ & $0.743^{+0.130}_{-0.328}$ & $-7.285^{+0.157}_{-0.149}$ & $3.318^{+0.051}_{-0.202}$ \\
% BurstySFH & $179485$ & $9.136^{+0.057}_{-0.069}$ & $8.037^{+0.104}_{-0.138}$ & $1.169^{+0.084}_{-0.090}$ & $-7.968^{+0.133}_{-0.123}$ & $2.952^{+0.050}_{-0.064}$ \\
% BurstySFH & $180446$ & $8.812^{+0.216}_{-0.471}$ & $8.341^{+0.128}_{-0.458}$ & $-0.492^{+0.635}_{-1.472}$ & $-9.366^{+1.123}_{-1.510}$ & $1.530^{+0.952}_{-0.711}$ \\
% BurstySFH & $300287$ & $8.708^{+0.095}_{-0.094}$ & $7.768^{+0.202}_{-0.049}$ & $1.228^{+0.066}_{-0.068}$ & $-7.480^{+0.114}_{-0.115}$ & $2.634^{+0.084}_{-0.084}$ \\
% BurstySFH & $300391$ & $7.969^{+0.091}_{-0.051}$ & $6.685^{+0.869}_{-0.466}$ & $1.225^{+0.097}_{-0.185}$ & $-6.746^{+0.111}_{-0.239}$ & $3.510^{+0.049}_{-0.061}$ \\
% BurstySFH & $380203$ & $7.714^{+0.352}_{-0.154}$ & $7.467^{+0.761}_{-1.210}$ & $0.883^{+0.063}_{-0.218}$ & $-6.825^{+0.191}_{-0.602}$ & $3.086^{+0.261}_{-0.125}$ \\

